MedicalRSI: Medical Recursive Self-Improving Agents via Clinical Model-Harness Co-Evolution

Medical agents built on large language models (LLMs) have advanced rapidly, yet most stay fixed once deployed and do not keep using their experience to improve later attempts. As a result, the same kind of error can recur across patients. To address this, existing self-improvement methods update an agent's weights or its medical harness from its own experience, but their improving strategy stays fixed and never learns which changes actually help, which caps how much the agent can improve. Recursive self-improvement (RSI) instead improves both the agent and its improving strategy. However, achieving RSI for medical agents is challenging, because clinical workflows rarely come with a reference harness, and a change that fixes early errors may not fix the problems the agent meets later. We propose MedicalRSI, an RSI framework built on Clinical Model-Harness Co-Evolution, in which one model plays two roles. The Solver is the medical agent itself, and the Improver is its learnable improving strategy, which writes a medical harness from the agent's failures. Each harness is rewarded by its gain over acting without it, and both roles are trained together, so the Improver keeps adapting to the problems the Solver has not yet solved. On multiple benchmarks and LLM backbones, MedicalRSI outperforms existing context-level and weight-level self-improvement methods and transfers well to unseen workflows, new LLMs and new databases, a step toward medical agents that keep improving.

==> figures/rendered/dims.tex <==
\makeatletter
\newcommand{\prerendered}[2]{\par\setbox\z@\hbox{\raisebox{-\csname figdp@#1\endcsname}{%
  #2}}\box\z@\vskip\csname figtrail@#1\endcsname\relax
  \prevdepth=\csname figpd@#1\endcsname\relax}
\@namedef{figdp@case_main}{78.04362pt}\@namedef{figtrail@case_main}{0.0pt}\@namedef{figpd@case_main}{78.04362pt}
\@namedef{figdp@case_app1}{118.59766pt}\@namedef{figtrail@case_app1}{0.0pt}\@namedef{figpd@case_app1}{118.59766pt}
\@namedef{figdp@case_app2}{98.61958pt}\@namedef{figtrail@case_app2}{0.0pt}\@namedef{figpd@case_app2}{98.61958pt}
\@namedef{figdp@case_app3}{98.61958pt}\@namedef{figtrail@case_app3}{0.0pt}\@namedef{figpd@case_app3}{98.61958pt}
\@namedef{figdp@case_app4}{142.2184pt}\@namedef{figtrail@case_app4}{0.0pt}\@namedef{figpd@case_app4}{142.2184pt}
\@namedef{figdp@case_app5}{164.28091pt}\@namedef{figtrail@case_app5}{0.0pt}\@namedef{figpd@case_app5}{164.28091pt}
\@namedef{figdp@case_app6}{118.57315pt}\@namedef{figtrail@case_app6}{0.0pt}\@namedef{figpd@case_app6}{118.57315pt}
\@namedef{figdp@case_tool1}{124.11292pt}\@namedef{figtrail@case_tool1}{0.0pt}\@namedef{figpd@case_tool1}{124.11292pt}
\makeatother

